An Empirical Study of Information Flows in Real-World JavaScript

Information flow analysis prevents secret or untrusted data from flowing into public or trusted sinks. Existing mechanisms cover a wide array of options, ranging from lightweight taint analysis to heavyweight information flow control that also considers implicit flows. Dynamic analysis, which is particularly popular for languages such as JavaScript, faces the question whether to invest in analyzing flows caused by not executing a particular branch, so-called hidden implicit flows. This paper addresses the questions how common different kinds of flows are in real-world programs, how important these flows are to enforce security policies, and how costly it is to consider these flows. We address these questions in an empirical study that analyzes 56 real-world JavaScript programs that suffer from various security problems, such as code injection vulnerabilities, denial of service vulnerabilities, memory leaks, and privacy leaks. The study is based on a state-of-the-art dynamic information flow analysis and a formalization of its core. We find that implicit flows are expensive to track in terms of permissiveness, label creep, and runtime overhead. We find a lightweight taint analysis to be sufficient for most of the studied security problems, while for some privacy-related code, observable tracking is sometimes required. In contrast, we do not find any evidence that tracking hidden implicit flows reveals otherwise missed security problems. Our results help security analysts and analysis designers to understand the cost-benefit tradeoffs of information flow analysis and provide empirical evidence that analyzing implicit flows in a cost-effective way is a relevant problem.

==> abstract.tex <==
Information flow analysis is widely used to enforce security policies that 
prevent sensitive data from flowing into untrusted sinks.
Security analysts face a wide range of options, ranging from lightweight 
taint analysis to heavyweight information flow analysis that also considers 
implicit flows.
Dynamic analysis, which is particularly popular for languages such as 
JavaScript, faces also the question whether to invest in analyzing flows 
caused by not executing a particular branch, which we call hidden implicit 
flows.
This paper addresses the questions how common implicit flows are in 
real-world programs, how important these flows are to enforce security 
policies, and what costs considering implicit flows involve.
We address these questions in an empirical study that analyzes over 
\lowerBoundEvents{} runtime events from \numberapps{} JavaScript programs 
with a state of the art dynamic information flow analysis.
The study shows that analyses that consider only a subset of all flows will 
miss violations of security policies. While taint analysis covers a fair 
amount of all violations (at least \percSSViolsFoundByTaint{}), it also 
misses a significant percentage (at least \percSSViolsMissedByTaint{}).  
Furthermore, we find a small but non-negligible number of policy violations 
caused by hidden implicit flows (\percSSFoundOnlyByHidden{}), which may leak 
sensitive data but are costly to analyze.
Our results help security analysts and analysis designers to understand the 
cost-benefit tradeoffs of information flow analysis and provide empirical 
evidence that analyzing implicit flows in a cost-effective way is a relevant 
problem.



==> background.tex <==
\section{Background}
\label{sec:background}

% policy
\paragraph*{Information flow policy}
An information flow analysis checks whether data from a sensitive 
\emph{source} influences data that arrives at an untrusted \emph{sink}.
Which parts of the program are considered to be sources and sinks is 
specified in an \emph{information flow policy}, or short, 
\emph{policy}.
\paragraph*{Propagation of security labels}
% labels
An information flow analysis associates each value with a \emph{security 
label} that indicates how secret the value is. Labels are typically 
arranged in a lattice~\cite{Denning1976}.
To ease the presentation, this paper focuses on two labels: $H$ (for high) 
and $L$ (for low), where $H$ is more secret than $L$.
% security stack, secret context
A dynamic information flow analysis identifies implicit flows by maintaining 
a \emph{security stack} that contains all $H$-labeled values that influence 
the control flow. When the stack is non-empty, the program executes in a 
\emph{secret context}.

 % monitoring strategies
\paragraph*{Monitoring strategies}
Different \emph{monitoring strategies} for dynamic information flow analysis 
address the problem of hidden implicit flows.
%
We build our work on the Permissive Upgrade (PU)~\cite{austin2010permissive}  
monitoring strategy, which is a refinement of the No Sensitive Upgrade 
strategy~\cite{austin2009efficient}.
These strategies terminate the execution of the program if an observable 
implicit flow may lead to a hidden implicit flow in another execution.
To this end, the PU strategy labels a value as \emph{partially leaked} if an 
$L$-labeled value is updated in a secret context, and terminates the program 
if the updated variable is further used outside the secret context.
For our example, consider again the execution where the password is 
``topSecret''. The PU strategy labels \code{gotIt} as partially leaked at 
line~\ref{line:write1} because the program writes to the $L$-labeled 
variable \code{gotIt} in a secret context, and terminates the program at 
line~\ref{line:sink}, because the value is used.

% upgrade statements
\paragraph*{Upgrade statements}
Naively applying the PU strategy to real-world programs is very restrictive 
and risks to terminate many executions.
To address this problem, Austin and Flanagan propose the \emph{upgrade 
statement}~\cite{austin2009efficient} or \emph{privatization 
statement}~\cite{austin2010permissive}. It changes the label of a variable 
to $H$, to signal a potential hidden implicit flow to the analysis.
%
For example, the highlighted upgrade statement at line~\ref{line:sink} of 
Figure~\ref{fig:example} marks \code{gotIt} as secret even if the branch is 
not taken.
As a result, the program does not terminate immediately when the value is 
read, but the information flow monitor finds a policy violation when the 
upgraded value is passed into the sink function \code{ajaxRequest}.



==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

This paper presents an empirical study of information flows in real-world 
programs.
Based on novel metrics to capture the prevalence of explicit, observable 
implicit, and hidden implicit flows, an automated methodology to apply these 
metrics, and manual inspection of a sample of flows, we study \numberapps{} 
JavaScript programs and thousands of security policies.
The results of our study show that all three kinds of flows are prevalent in 
practice, and that not considering some of them may cause an analysis to 
miss leaks of sensitive information.
At the same time, we find that a lightweight taint analysis must consider 
significantly fewer runtime operations but can still find many violations of 
security policies.
Our work helps security analysts and analysis developers to better 
understand the tradeoffs involved in designing an information flow analysis.  
Furthermore, our findings highlight the need for future research on 
cost-effective ways to analyze both observable and hidden implicit 
information flows.



==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

To implement the methodology described in the previous section, we implement 
a dynamic information flow analysis 
following~\cite{Hedin2012,hedin2014jsflow}. The implementation builds on 
Jalangi~\cite{Sen2013}, a dynamic analysis framework for JavaScript that 
uses source-to-source transformation.  To approximate the effects of native 
calls, we model them as transferring the labels from all parameters to the 
return value.
The runtime analysis writes the iFlow trace to the file system, and the 
metrics are computed offline, i.e., after the execution.
When inserting upgrades, the implementation does not modify the actual 
source code but stores the source code locations of upgrades and performs 
the upgrades at runtime.




==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

%% info flow analysis is important
Analyzing and enforcing a security policy for a program is important to 
prevent sensitive data from leaking to untrusted sinks.
For example, a user may want to allow a browser extension to keep track of 
mouse movements but disallow sending this information to a third party.
One way to enforce security policies is \emph{information flow 
analysis}, which keeps track of how secrets propagate through a 
program~\cite{Denning1976,Sabelfeld2003}.

%% there are different kinds of flows
Even though there is consensus that analyzing information flows is 
important, there is a range of options regarding the kinds of flows to 
consider.
As a coarse-grained classification, there are two kinds of flows:  
\emph{explicit flows}, caused by computing new data from existing secret 
data, and \emph{implicit flows}, caused by control flow decisions that 
depend on secret data.
For a dynamic information flow analysis, the second kind can be further 
classified into flows that happen because a particular branch is executed, 
which we call \emph{observable implicit flows}, and flows that happen 
because a particular branch is not executed, which we call \emph{hidden 
implicit flows}.\footnote{There are other kinds of flows, such as timing 
side-channels and cache side-channels, which we ignore in this paper.}
All three kinds of flows can cause sensitive data to leak to an untrusted 
sink, and ideally, an information flow analysis considers all of them.

%% illustrate hidden implicit flow
\begin{figure}
\begin{spacing}{0.9}
\begin{lstlisting}
var gotIt = false;
var passwd = ...;
// mark as secret:
/*#\HL#*/markSource(passwd);/*#\HLoff#*//*#\label{line:markSource}#*/
var paddedPasswd = "xx" + passwd;/*#\label{line:explicit}#*/
var knownPasswd = null;
if (paddedPasswd === "xxtopSecret") {/*#\label{line:cond}#*/
  gotIt = true;/*#\label{line:write1}#*/
  knownPasswd = passwd;/*#\label{line:write2}#*/
}/*#\label{line:merge}#*/
// mark as untrusted:
/*#\HL#*/markSink(ajaxRequest);/*#\HLoff#*//*#\label{line:markSink}#*/
ajaxRequest("evil.com", /*#\HL#*/upgrade(/*#\HLoff#*/gotIt /*#\HL#*/)/*#\HLoff#*/);/*#\label{line:sink}#*/
\end{lstlisting}
\end{spacing}
\caption{Example program that leaks the password to the network. The meaning 
of \code{upgrade} will be explained in Section~\ref{sec:background}.}
\label{fig:example}
\end{figure}

Figure~\ref{fig:example} shows a simple JavaScript program that illustrates 
the different kinds of flows and how they may leak sensitive information. 
The program has a variable \code{passwd}, which is marked as a secret at 
line~\ref{line:markSource}.
Using this variable in an operation that creates a new value, e.g., in 
line~\ref{line:explicit}, is an explicit flow.
%
Consider the case where the password is ``topSecret'', i.e., the conditional 
at line~\ref{line:cond} evaluates to \code{true}, and line~\ref{line:write1} 
sets \code{gotIt} to \code{true}.
At line~\ref{line:sink}, the \code{gotIt} variable is sent to the network 
through the function \code{ajaxRequest()}, which is considered to be an 
untrusted sink. The flow from the password to \code{gotIt} is an observable 
implicit flow because a secret value determines that \code{gotIt} gets 
written.
%
Now, consider the case where the password is ``abc''. In this case, the 
branch at line~\ref{line:cond} is not taken and the \code{gotIt} variable 
remains \code{false}. Sending this information to the network reveals that 
the password is different from ``topSecret''. This flow is a hidden implicit 
flow because a secret value determines that \code{gotIt} gets not written.

\begin{table}
  \caption{\todo{Remove duplicates} Recent information flow analyses and the 
  kinds of flows they support (\checkmark means the analysis considers this 
  flow, \text{\sffamily -} means the analysis does not consider this flow,  
  \text{\sffamily x} means the flow is prevented by terminating the 
  program).}
  \setlength{\tabcolsep}{1.2pt}
  \renewcommand{\arraystretch}{0.8}
    \begin{tabular}{@{}lllccc@{}}
	\toprule
  &&&\multicolumn{3}{@{}c@{}}{Supported Flows} \\
  \cmidrule{4-6}
  &&&&\multicolumn{2}{@{}c@{}}{Implicit} \\
  \cmidrule{5-6}
  Work & Analysis & Language & Explicit &  Observable & Hidden \\
    \midrule
    \cite{Chudnov:2015:IIF:2810103.2813684} & dynamic & JavaScript & \checkmark & \checkmark  & \text{\sffamily x}  \\
    \cite{bastaniinteractively} & static & Java &  \checkmark & 
    \text{\sffamily -} & \text{\sffamily -}\\    \cite{hedin2015}& static + 
    dyn. & JavaScript & \checkmark & \checkmark & \checkmark\\    
    \cite{rajani2015information} & dynamic & JavaScript & \checkmark & 
    \checkmark & \text{\sffamily x}\\
    \cite{bauer2015run} & dynamic & JavaScript & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
    \cite{ming2015taint} & dynamic & hardware & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
    \cite{askarov2015hybrid} & static + dyn. & theoretical & \checkmark & 
    \checkmark & \checkmark \\  \cite{bauer2015run} & dynamic & JavaScript / 
    C & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
	\cite{gordon2015information} & static & Java & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
    \cite{bastaniinteractively} & static & Java & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
    \cite{cox2014spandex} & dynamic & Java & \checkmark & \checkmark & \checkmark\\
    \cite{buiras2014dynamic} & dynamic & JavaScript & \checkmark & \checkmark & \checkmark\\
    \cite{arzt2014flowdroid} & static & Java & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
    \cite{dahse2014simulation} & static & PHP & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\
    \cite{sun2014detecting} & static & PHP & \checkmark & \text{\sffamily -} & \text{\sffamily -}\\     
   % \cite{Lekies:2013:MFL:2508859.2516703} & dynamic & JavaScript & \checkmark & \text{\sffamily -} & \text{\sffamily -} \\ 

	\bottomrule
  \end{tabular}
  \label{tab:recent-work}
\end{table}

%% tracking flows has a cost -- tradeoff
Tracking flows of information comes at computational and human costs.
For example, dynamically tracking implicit flows imposes a higher runtime 
overhead than tracking only explicit flows, and dynamically detecting hidden 
implicit flows~\cite{austin2009efficient} requires the program to be 
augmented with so called \emph{upgrade} statements.
%
Because of these costs, many analyses consider only a subset of all flows. 
Table~\ref{tab:recent-work} surveys some recent approaches.  Many analyses, 
often called taint analyses, consider only explicit flows.  Among the 
analyses that consider implicit flows, some stop the program as soon as a 
hidden flow occurs.

%% is this effort worth it? answering this question is important
Given the costs of tracking implicit information flows, it is important to 
ask how relevant the problem of implicit flows is.
Specifically, we ask the following research questions:
\begin{itemize*}
  \item RQ1: How many of all operations that induce an information flow are 
    explicit flows, observable implicit flows, and hidden implicit flows,    
    respectively?

  \item RQ2: How much do the different kinds of flows contribute to the 
    detection of violations of security policies?

  \item RQ3: Do implicit flows that cause a violation of an information flow 
    policy propagate important data?

  \item RQ4: What is the cost, both computational and human, of considering 
    implicit flows in addition to explicit flows?

  \item RQ5: What is the influence of the information flow policy, i.e., 
    which data is marked as sensitive and which locations are considered as 
    untrusted sinks, on the prevalence of the different kinds of flows? 
  
\end{itemize*}
Answering these questions will provide evidence to support or refute 
assumptions about the importance of particular kinds of flows.
%
%% discuss closest existing work
Prior work studies false positives caused by static analysis of implicit 
flows~\cite{King2008} and the semantic strength of 
flows~\cite{masri2009measuring}. However, to the best of our knowledge, no 
existing work addresses the above questions.

To address our research questions, this paper presents an empirical study of 
information flows in real-world JavaScript programs. The study involves 
\numberapps{} programs and that yield over \lowerBoundEvents{} information 
flow-related runtime events.
Our study is enabled by a novel methodology that combines state of the art 
dynamic information flow 
analysis~\cite{Hedin2012,hedin2014jsflow,austin2010permissive} and program 
rewriting~\cite{birgisson2012boosting} with a set of novel metrics to 
measure the prevalence of different kinds of flows and the cost of tracking 
them.
Large parts of the methodology are language-independent, making it easily 
applicable to languages other than JavaScript.
The approach consist of a language-dependent online analysis, which 
summarizes an execution into an information flow-specific trace, and a 
language-independent offline analysis, which implements the metrics required 
to address our research questions and provides a formal basis to address 
additional questions.

%% summarize results
The main findings of our study are the following:
\begin{itemize*}
  \item All three kinds of flows occur in practice, i.e., an analysis that 
    ignores some of them risks to miss violations of the information flow 
    policy.  (RQ1)
  \item Observable implicit flows and explicit flows are the most prevalent, 
    accounting for \percObsImplMicroFlows{} and \percExplMicroFlows{} of all 
    flows, respectively.
    (RQ1)
  \item A lightweight taint analysis can detect a significant amount     (at 
    least \percSSViolsFoundByTaint{}) of violations of security policies, 
    but also misses several of them (at least \percSSViolsMissedByTaint{}).  
    (RQ2)
  \item An analysis that considers explicit and observable implicit flows, 
    but ignores hidden implicit flows, detects most violations (at least 
    \percSSFoundByAllButHidden{}). (RQ2)
  \item Most implicit flows do not convey security-critical information but 
    harmless data, such as whether a property is defined or what type a 
    variable has.  As a result, none of the policy violations that involve 
    implicit flows corresponds to a security vulnerability.  This finding 
    suggests that implicit flows are less important than explicit flows, at 
    least for the programs and policies used in the study. (RQ3)
  \item The computational cost of considering implicit flows is significant: 
    Ignoring implicit flows saves the effort of tracking 
    \percEventsExplicitOnly{} of all runtime operations. (RQ4)
  \item The human cost of analyzing implicit flows, in particular, the cost 
    of adding annotations and inspecting potential vulnerabilities, is 
    manageable for most applications. (RQ4)
  \item The information flow policy has a huge impact on the prevalence of 
    different kinds of flows. (RQ5)
\end{itemize*}

As one might expect, our results do not provide a simple answer to the 
question from the paper's title. We show that taint analysis covers a 
significant percentage of flows and policy violations, and that full 
information flow analysis comes at a non-negligible cost that may not pay 
off proportionally.

%% summary of contributions
In summary, this paper contributes the following:
\begin{itemize*}
  \item We are the first to empirically study the prevalence of explicit, 
    observable implicit, and hidden implicit information flows in real-world 
    software.
  \item We present a methodology that enables the study and that provides a 
    formal basis for studying information flows in a programming 
    language-independent way.
  \item We provide empirical evidence that sheds light on the cost-benefit 
    tradeoffs of information analysis and that outlines directions for 
    future work.
\end{itemize*}



==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}

To address the research questions from Section~\ref{sec:intro}, we present a 
methodology that combines a set of novel metrics with a dynamic information 
flow analysis~\cite{Hedin2012,hedin2014jsflow}, a monitoring 
strategy~\cite{austin2010permissive}, and an automated mechanism to insert 
upgrade statements~\cite{birgisson2012boosting}.
The metrics we present summarize flows observed during the execution of the 
program, with the goal to measure the prevalence of flows.  This goal is in 
contrast to typical runtime monitors that terminate the program when an 
information flow policy is violated. Instead, we continue the execution even 
after a policy violation to measure flows in the remainder of the execution.
%
The methodology consists of an online part, which gathers a trace of 
information flow-related runtime events (Section~\ref{sec:traceLanguage}), 
and an offline part, which extracts answers to our research questions 
(Section~\ref{sec:metrics}).
To prepare the program for the analysis, the approach repeatedly executes 
it while inserting all required upgrade statements  
(Section~\ref{sec:onlinePhase}).


% MP: Removed the figure because we are short in space.
%     If we include it, we should revise it (e.g., to include iFlow trace).
%\begin{figure}
%\centering
%\epsfig{file=res/workflow.pdf, height=1.2in, width=3.7in}
%\caption{The main steps of our methodology, split into two phases. }
%\label{fig:high-level}
%\end{figure}
%
%Figure~\ref{fig:high-level} gives an overview of our methodology. Given a 
%program, tests that exercise the program, and an information flow policy, 
%the approach goes through an \textit{online} phase and an \textit{offline} 
%phase to eventually produce results that address our research questions. We 
%explain the different parts of the approach in the following, starting with 
%the information flow trace, which connects the two phases with each other.

\begin{figure}[tb]
\begin{grammar}
<Stmt> ::= markSrc(x) | x=y | x[y]=z | x=y~$\diamond$~z \alt
if (x) \{ $\overline{s}$ \} | while (x) \{ $\overline{s}$ \} | f(x) | 
markSink(f)
\end{grammar}

\vspace{.5em}
$\begin{array}{l}
  x,y,z,f \in \mbox{Name}\\
  a \in \mbox{Address}\\
  u \in \mbox{Value} \\
  \rho \in \mbox{Env} := \mbox{Name} \rightharpoonup \mbox{Value}\\
  h \in \mbox{Heap} := \mbox{Address} \rightharpoonup \mbox{Rec}\\
  r \in \mbox{Rec} ::= \{ \overline{x:~u} \}\\
\end{array}$
\caption{Grammar and semantic domains of nanoJS, a core of JavaScript.}
\label{fig:JSlang}
\end{figure}

We formally describe our methodology for a simple, JavaScript-inspired core 
language, called nanoJS.  Our implementation supports the entire JavaScript 
language; we focus the description on nanoJS to ease the presentation.
Figure~\ref{fig:JSlang} defines the syntax of nanoJS and its semantic 
domains. The language includes only features that are relevant for answering 
our research questions.
Beyond standard features, the language contains a \code{markSrc(x)} 
statement, which marks a value as sensitive information, and a 
\code{markSink(f)} statement, which marks a function as a sink.


\subsection{Gathering an Information Flow Trace}
\label{sec:traceLanguage}


To reason about different kinds of information flows, we present a trace 
language called iFlow. The language summarizes  information flow-related 
operations into a format that abstracts from details of the programming 
language. As a result, we can define metrics to answer our research 
questions in a concise and language-independent way. We design iFlow to 
provide a formal basis for addressing not only our but also other research 
questions.


\subsubsection{Language Definition}

\begin{figure}
\begin{grammar}
<Trace> ::= <Event>

%\vspace{-2mm}
<Event> ::=
<Event>\;;\;<Event> \alt
<ProgramEvent> \alt
<PolicyEvent>

%\vspace{-2mm}
<ProgramEvent> ::= write($v_{old}$, $v_{new}$) \alt
operation($v_1$, $v_{new}$) \alt
operation($v_1$, $v_2$, $v_{new}$) 

%\vspace{-2mm}
<PolicyEvent> ::= source($v$, $l_{src}$) \alt
sink($v$, $l_{snk}$) \alt
upgrade($v_{old}$, $v_{new}$, $l_{src}$) \alt
push($v$) ; <Event> ; pop 

%\vspace{-2mm}

\vspace{.5em}
<$v$, $v_{old}$, $v_{new}$, $v_1$, $v_{2}$> $\in$ <ValueIds>

\vspace{-2mm}
<$l_{src}$, $l_{snk}$> $\in$ <SourceLocs>
%\vspace{-2mm}
\end{grammar}
\caption{Grammar of the iFlow language for describing information flow 
traces.}
\label{fig:lang}
\end{figure}

Figure~\ref{fig:lang} gives the grammar of the iFlow language.
A trace is a sequence of runtime events.
Each runtime value is represented by a unique identifier, i.e., the trace 
does not store the values themselves. The iFlow language considers values to 
be immutable and creates new unique value identifiers whenever a value or 
its security label changes.

We distinguish two kinds of events. First, \emph{program events} represent 
the behavior of the original program.  The $write$ event represents a write 
to a variable or a property, where $v_{old}$ is overwritten by $v_{new}$.
The $operation$ events represent unary and binary operations, such as 
arithmetic operations, where $v_{new}$ is created from one or two existing 
values.
The language omits other program events, such as variable reads, because 
they do not cause any information flow.

Second, \emph{policy events} represent the behavior of the  information flow 
analysis.
The $source$ event represents that a value is marked as a source, which 
yields a new value $v$ with security label $H$.
The $sink$ event represents that $v$ flows into a sink function.  Both 
$source$ and $sink$ events are associated with a code location $l_{src}$ and 
$l_{snk}$, respectively.
The $upgrade$ event represents that $v_{old}$ gets upgraded into the 
$H$-labeled $v_{new}$; it is also associated with the corresponding code 
location, $l_{src}$.
Furthermore, the language has $push$ and $pop$ events that represent updates 
of the security stack.


\subsubsection{Abstracting an Execution into iFlow}

\newcommand{\ruleDist}{.5em}
\setpremisesend{0em}
\setpremisesspace{.7em}
\begin{figure}[tb]
  \[ \inference[\textsc{\scriptsize(source)}]
{
  \rho(x)=u &
  reachable(u)=\{u_0,...,u_n\} \\
  \iota(u_k) = v_k~\forall k \in 0..n
}
{
  <markSrc(x), h, \rho, \iota, \kappa>
  |/
  <source(v_0);...;source(v_n)>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(assign)}]{
  \kappa(\rho(y))=H &
  v_{new} = \iota(\rho(y)) \\
  v_{old} = \left\{
    {\begin{array}{ll}
      \bot & \mbox{if } x \notin dom(\rho) \vee \kappa(\rho(x))=L \\
      \iota(\rho(x)) & \mbox{otherwise}
    \end{array}}
  \right.
}
{
  <x=y, h, \rho, \iota, \kappa>
  |/
  <write(v_{old}, v_{new})>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(store)}]{
  \kappa(\rho(z))=H &
  \rho(x)=a &
  h(a)=r &
  \rho(y)=y' \\
  v_{old} = \left\{
    {\begin{array}{ll}
      \bot & \mbox{if } y' \notin dom(r) \vee \kappa(r(y'))=L \\
      \iota(r(y')) & \mbox{otherwise}
    \end{array}}
  \right. \\
  v_{new}=\iota(\rho(z))
}
{
  <x[y]=z, h, \rho, \iota, \kappa>
  |/
  <write(v_{old}, v_{new})>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(op)}]
{
  \kappa(\rho(y))=H \vee \kappa(\rho(z))=H &
  v_1 = \iota(\rho(y)) &
  v_2=\iota(\rho(z)) \\
  u_{new} = \rho(y) |[ \diamond |] \rho(z) &
  v_{new}=\iota(u_{new})
}
{
  <x=y \diamond z, h, \iota, \kappa>
  |/
  <operation(v_1, v_2, v_{new})>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(if$_T$)}]
{
  \kappa(\rho(x))=H &
  \rho(x) = True &
  v_x=\iota(\rho(x)) \\
  < \overline{s}, h, p, \iota, \kappa> |/ <t>
}
{
  <if(x) \{ \overline{s} \}, h, \rho, \iota, \kappa>
  |/
  <push(v_x); t; pop>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(if$_F$)}]
{
  \rho(x) = False
}
{
  <if(x) \{ \overline{s} \}, h, \rho, \iota, \kappa>
  |/
  <\epsilon>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(while)}]
{
  <if (x) \{ \overline{s}; while(x) \{ \overline{s} \}\}, h, \rho, \iota, 
  \kappa>
  |/
  <t>
}
{
  <while(x) \{ \overline{s} \}, h, \rho, \iota, \kappa>
  |/
  <t>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(upgrade)}]
{
  \kappa(\rho(x))=L &
  v_{old}=\iota(\rho(x)) \\
  v_{new}=\iota( |[ upgrade(x) |] )
}
{
  <upgrade(x), h, \rho, \iota, \kappa>
  |/
  <upgrade(v_{old}, v_{new})>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(sink)}]
{
  \mathcal{H}=\{ u ~\vert~ u \in reachable(\rho(x)) \wedge \kappa(u)=H\} \\
  f \mbox{~is a sink} &
  \vert \mathcal{H} \vert = n \geq 1 &
  \iota(u_k)=v_k~\forall k \in 0..n
}
{
  <f(x), h, \rho, \iota, \kappa>
  |/
  <sink(v_0);...;sink(v_n)>
} \]

\caption{Operational semantics for creating an iFlow execution trace.}
\label{fig:semanticsCreateTrace}
\end{figure}


To obtain an iFlow trace, we augment dynamic information flow analysis to 
record runtime events.
The trace omits all runtime operations that operate only on $L$-labeled 
data.
%
Figure~\ref{fig:semanticsCreateTrace} summarizes how the analysis creates an 
iFlow trace from a nanoJS execution, using big-step operational semantics of 
nanoJS.
The semantics is a transition system that evaluates (written as 
$\Downarrow$) statements into iFlow trace entries. Each evaluation step 
transforms a state $<s,h,\rho,\iota,\kappa>$ into a state $<t>$, where $s$ 
is a nanoJS statement, $h$ is the heap, $\rho$ is the environment that maps 
variables to values, and $t$ is a trace event.
The maps $\iota: Value \rightarrow ValueId$ and $\kappa: Value \rightarrow 
\{L, H\}$ assign to each value a unique identifier and the value's security 
label, respectively.
%
To simplify the presentation, we include neither the semantics of the normal 
nanoJS execution, which follows the JavaScript semantics, nor the semantics 
of the information flow analysis, i.e., how to create and propagate labels, 
which follows~\cite{Hedin2012,hedin2014jsflow}.
%
Moreover, Figure~\ref{fig:semanticsCreateTrace} omits that trace entries are 
labeled with their source location.

When the program marks a variable $x$ as a source, then the analysis records 
a $source$ event for each value reachable from $x$ (rule \textsc{\small 
src}).  %
For writes into a variable or an object property, the analysis records a 
$write$ event (rules \textsc{\small assign} and \textsc{\small store}).
The $write$ event refers to the old, overwritten value and to the newly 
written value. If the old value is $L$-labeled or not defined, then the 
analysis records $\bot$ instead.
%
For binary operations $\diamond$, such as arithmetic operations, where at 
least one input value is $H$-labeled, the approach records an $operation$ 
event (rule \textsc{\small op}).
The result value is computed according to the standard semantics of 
JavaScript and the information flow analysis, indicated by $|[ \diamond |]$. 
The rule for unary operations is similar and therefore omitted.

To maintain the security stack, the analysis records a $push$ event for each 
$H$-labeled conditional that evaluates to \code{true} (rules \textsc{\small 
if$_F$}, \textsc{\small if$_T$}, and \textsc{\small while}).  At the end of 
the block guarded by that conditional, the analysis records a $pop$ event.
%
For upgrade statements, the analysis checks whether the value is $L$-labeled 
before the upgrade, and if so, records an $upgrade$ event (rule 
\textsc{\small upgrade}).
%
Finally, when the program passes a value $x$ to a sink function, then the 
analysis generates a $sink$ event for each secret value reachable from $x$ 
(rule \textsc{\small sink}).


\resetCtr{}
\begin{figure}
  \small
  \renewcommand{\arraystretch}{1.1}
  \setlength{\tabcolsep}{2.1pt}
  \begin{tabular}{@{}rlccccc@{}}
\toprule
Id & Event & \multicolumn{5}{c}{Interpretation (state after the event)} \\
\cmidrule{3-7}
& & $\mathcal{S}$ & $t$ & \multicolumn{3}{c}{Micro flow counters} \\
\cmidrule{5-7}
& & & & Expl. & Obs. & Hid. \\
\midrule
\nextCtr{} & $source(v_2, \mbox{line~\ref{line:markSource}})$ &
$\{v_2\}$ & $[]$ & 0 & 0 & 0 \\
\nextCtr{} & $operation(v_3, v_2, v_4)$ &
$\{v_2,v_4\}$ & $[]$ & 0 & 0 & 0 \\
\nextCtr{} & $write(\bot, v_4)$ &
$\{v_2,v_4\}$ & $[]$ & 1 & 0 & 0 \\
\nextCtr{} & $operation(v_4, v_6, v_7)$ &
$\{v_2,v_4,v_7\}$ & $[]$ & 1 & 0 & 0 \\
\nextCtr{} & $push(v_7)$ &
$\{v_2,v_4,v_7\}$ & $[v_7]$ & 1 & 0 & 0\\
\nextCtr{} & $write(v_1, v_8)$ &
$\{v_2,v_4,v_7,v_8\}$ & $[v_7]$ & 1 & 1 & 0\\
\nextCtr{} & $write(v_5, v_2)$ &
$\{v_2,v_4,v_7,v_8\}$ & $[v_7]$ & 2 & 2 & 0\\
\nextCtr{} & $pop$ &
$\{v_2,v_4,v_7,v_8\}$ & $[]$ & 2 & 2 & 0\\
\nextCtr{} & $sink(v_9, \mbox{line~\ref{line:sink}})$ &
$\{v_2,v_4,v_7,v_8\}$ & $[]$ & 2 & 2 & 0\\
\bottomrule
  \end{tabular}

  \vspace{.2em}
  \begin{spacing}{0.8}
Values:
$v_1=\mbox{false}^L$,
$v_2=\mbox{``topSecret''}^H$,
$v_3=\mbox{``xx''}^L$,
\mbox{$v_4=\mbox{``xxtopSecret''}^H$},
$v_5=\mbox{null}^L$,
$v_6=\mbox{``xxtopSecret''}^L$,
\mbox{$v_7=\mbox{true}^H$},
$v_8=\mbox{true}^H$,
$v_9=\mbox{true}^H$,
%
$\bot=\mbox{non-existing value}^L$
\end{spacing}
  \caption{Trace of execution with password ``topSecret''.}
  \label{fig:traceBranchTaken}
\end{figure}

\resetCtr{}
\begin{figure}
  \small
  \renewcommand{\arraystretch}{1.1}
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{@{}rlccccc@{}}
\toprule
Id & Event & \multicolumn{5}{c}{Interpretation (state after the event)} \\
\cmidrule{3-7}
& & $\mathcal{S}$ & $t$ & \multicolumn{3}{c}{Micro flow counters} \\
\cmidrule{5-7}
& & & & Expl. & Obs. & Hid. \\
\midrule
\nextCtr{} & $source(v_2, \mbox{line~\ref{line:markSource}})$ &
$\{v_2\}$ & $[]$ & 0 & 0 & 0 \\
\nextCtr{} & $operation(v_3, v_2, v_4)$ &
$\{v_2\}$ & $[]$ & 0 & 0 & 0 \\
\nextCtr{} & $write(\bot, v_4)$ &
$\{v_2,v_4\}$ & $[]$ & 1 & 0 & 0 \\
\nextCtr{} & $operation(v_4, v_5, v_6)$ &
$\{v_2,v_4,v_6\}$ & $[]$ & 1 & 0 & 0 \\
\nextCtr{} & $upgrade(v_1, v_7, \mbox{line~\ref{line:sink}})$ &
$\{v_2,v_4,v_6,v_7\}$ & $[]$ & 1 & 0 & 1\\
\nextCtr{} & $sink(v_7, \mbox{line~\ref{line:sink}})$ &
$\{v_2,v_4,v_6,v_7\}$ & $[]$ & 1 & 0 & 1\\
\bottomrule
  \end{tabular}

  \vspace{.2em}
  \begin{spacing}{0.8}
Values:
$v_1=\mbox{false}^L$,
$v_2=\mbox{``abc''}^H$,
$v_3=\mbox{``xx''}^L$,
$v_4=\mbox{``xxabc''}^H$,
$v_5=\mbox{``xxtopSecret''}^L$,
$v_6=\mbox{false}^H$,
$v_7=\mbox{false}^H$,
%
$\bot=\mbox{non-existing value}^L$
\end{spacing}
  \caption{Trace of execution with password ``abc''.}
  \label{fig:traceBranchNotTaken}
\end{figure}

For example, the first two columns of Figure~\ref{fig:traceBranchTaken} show 
the information flow trace of an execution of Figure~\ref{fig:example} where 
the password is ``topSecret''.
The trace contains $push$ and $pop$ events to indicate that 
lines~\ref{line:write1} and~\ref{line:write2} the program executes in a 
secret context. Figure~\ref{fig:traceBranchNotTaken} shows a trace generated 
by an execution with password ``abc'', i.e., an execution where the branch 
is not taken.
Because this execution does not take the branch, the trace contains no 
$push$ and $pop$ events.
The bottom of both figures show all values involved in the execution, along 
with the unique value identifier and the security label of each value.


\subsection{Measuring the Prevalence of Flows}
\label{sec:metrics}

Based on an iFlow trace, the approach measures the prevalence of different 
kinds of information flows.
The basic idea is to iterate through the trace while incrementing counters 
that represent the number of explicit, observable implicit, and hidden 
implicit flows.
We consider information flows at two levels of granularity.
On the one hand, we consider flows induced by a single event in the trace, 
i.e., by a single operation in the program 
(Section~\ref{sec:metricsMicroFlows}).  We call such flows \emph{micro 
flows} or simply flows.
Studying flows at the micro flow level is worthwhile because it provides a 
detailed understanding of the operations that contribute to higher-level 
flows.
On the other hand, we consider transitive flows of data between a source and 
a sink, called \emph{source-to-sink flows} (Section~\ref{sec:S2SFlows}).
Studying flows at this coarse-grained level is worthwhile because 
source-to-sink flows are what security analysts are ultimately interested in 
when using an information flow analysis.

The metrics presented in this section measure the prevalence of flows 
quantitatively, and do not attempt to judge the importance of flows. To 
understand the importance of individual flows, we manually 
inspect a subset of all flows (Section~\ref{sec:importanceOfIF}).

While traversing the trace, the approach maintains a set $\mathcal{S}$ of 
values that are known to be secret. We call this set the \emph{tagged 
values}. Once a value is tagged, it cannot be removed from $\mathcal{S}$ 
anymore. Tagging a value while interpreting an iFlow trace is roughly 
equivalent to marking a value with label $H$ while the program executes. We 
introduce a new terminology to avoid confusion between the description of 
how an iFlow trace is created and how it is interpreted.


\subsubsection{Micro Flows}
\label{sec:metricsMicroFlows}

To measure how many explicit, observable implicit, and hidden implicit 
flows exist, our approach increments the respective counters for these micro 
flows as follows.

\paragraph*{Explicit flows}
The approach counts an explicit flow for every \emph{write} event where the 
written value is tagged but the value that gets overwritten (if any) is not 
tagged. The rationale is to capture program behavior where secret 
information flows to a memory location that has not stored such information 
before. In contrast, overwriting a secret value with another secret value 
does not leak any new information, and therefore does not count as an 
explicit flow.
    
    For example, consider this code:
\begin{lstlisting}
var x = 3; var y = 5; var z;
markSrc(x);
markSrc(y);
x = y; // no explicit flow
z = x; // explicit flow
\end{lstlisting}

\paragraph*{Observable implicit flows}
The approach counts an observable implicit flow for every $write$ event that 
happens in a secret context and that overwrites a non-tagged value.  Similar 
to explicit flows, the rationale is to capture program behavior that writes 
secret information to a memory location that has not stored such information 
before. The main difference is that the write happens because of a control 
flow decision made based on a secret value.  Note that it is irrelevant 
whether the written value is tagged because the fact that a write happens 
leaks secret information.

For example, consider this code:
\begin{lstlisting}
var x = true; var y = 3; var z;
markSrc(x);
if (x)
  y = 5; // observable implicit flow
z = 7;   // no flow
\end{lstlisting}

\paragraph*{Hidden implicit flows}
The approach counts a hidden implicit flow for every $upgrade$ event. The 
rationale is to capture write operations that did not happen, but that could 
have happened during the execution if a control flow decision that depends 
on a secret value would have been different.
Since the approach creates such an $upgrade$ event only if the upgraded 
value has not been secret before the upgrade 
(Section~\ref{sec:traceLanguage}), the trace interpreter need not check this 
condition again.

For example, consider this code:
\begin{lstlisting}
var x = false; var y; var z;
markSrc(x);
if (x)
  y = 5;        // not executed, no flow
z = upgrade(y); // hidden implicit flow
\end{lstlisting}


%\begin{mydef}
%  \label{def:ef}
%  An {\bfseries explicit flow} occurs when there is an event $write(v_{old}, 
%  v_{new})$ where $v_{old}$ is $L$-labeled and where $v_{new}$ is 
%  $H$-labeled.
%\end{mydef}
%
%\begin{mydef}
%Let $t$ be the stack maintained by interpreting the $push$ and $pop$ events 
%in a trace.
%An {\bfseries observable implicit flow} occurs when there is an event 
%$write(v_{old}, v_{new})$ while $t$ is non-empty and where $v_{old}$ is 
%$L$-labeled.
%\end{mydef}
%
%\begin{mydef}
%\label{def:hif}
%A {\bfseries hidden implicit flow} occurs when there is an event 
%$upgrade(v_{old},v_{new}, *)$ where $v_{old}$ is $L$-labeled.
%\end{mydef}

\begin{figure}[tb]
\[ \inference[\textsc{\scriptsize(src)}] {
  e = source(v)
}
{
  <e, \mathcal{S}, t, c_E, c_O, c_H>
  |/
  <\mathcal{S} \cup \{v\}, t, c_E, c_O, c_H>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(write)}] {
  e = write(v_{old}, v_{new}) \\
  c_E' = \left\{
    {\begin{array}{ll}
      c_E + 1 & \mbox{if } v_{old} \notin \mathcal{S} \wedge v_{new} \in 
      \mathcal{S} \\
      c_E & \mbox{otherwise}
    \end{array}}
  \right. \\
  c_O' = \left\{
    {\begin{array}{ll}
      c_O + 1 & \mbox{if } v_{old} \notin \mathcal{S} \wedge t \neq 
      \mbox{empty} \\
      c_O & \mbox{otherwise}
    \end{array}}
  \right.
}
{
<e, \mathcal{S}, t, c_E, c_O, c_H>
  |/
  <\mathcal{S} \cup \{ v_{new} \}, t, c_E', c_O', c_H>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(op)}] {
  e = operation(v_1,v_2,v_{new}) &
}
{
<e, \mathcal{S}, t, c_E, c_O, c_H>
  |/
  <\mathcal{S} \cup \{v_{new}\}, t, c_E, c_O, c_H>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(stack)}] {
  e_{push} = push(v) &
  t' = v \circ t \\
  <e, \mathcal{S}, t', c_E, c_O, c_H>
  |/ <\mathcal{S}', t'', c_E', c_O', c_H'>
}
{
  <e_{push}; e; pop, s, t, c_E, c_O, c_H>
  |/
  <\mathcal{S}', t, c_E', c_O', c_H'>
} \]

\vspace{\ruleDist{}}

\[ \inference[\textsc{\scriptsize(upgrade)}] {
  e=upgrade(v_{old}, v_{new}) &
  c_H' = c_H + 1
}
{
<e, \mathcal{S}, t, c_E, c_O, c_H>
  |/
  <\mathcal{S} \cup \{v\}, t, c_E, c_O, c_H'>
} \]
\caption{Operational semantics of interpreting an iFlow trace.}
\label{fig:semanticsInterpretTraceMicroFlows}
\end{figure}

We formally describe how to measure micro flows by giving the big step 
operational semantics of iFlow 
(Figure~\ref{fig:semanticsInterpretTraceMicroFlows}).
The semantic rules evaluate a state $<e, \mathcal{S}, t, c_E, c_O, c_H>$ 
into a state $<\mathcal{S}, t, c_E, c_I, c_H>$, where $e$ is an iFlow event,
$\mathcal{S} \subseteq \mbox{ValueId}$ represents the set of tagged values, 
$t$ is the security stack, and $c_E, c_O, c_H$ are the counters of explicit, 
observable implicit, and hidden implicit flows, respectively.

Events $source$, $write$, $operation$, and $upgrade$ all result in a secret 
value and therefore tag this value by adding it to $\mathcal{S}$.
%
A $write$ event increments the number $c_E$ of explicit flows if and only if 
the overwritten value $v_{old}$ is not yet tagged but the written value 
$v_{new}$ is tagged (rule \textsc{\small write}).
If the security stack $t$ is non-empty and if the overwritten value is not 
tagged, then the $write$ event also increments the number $c_O$ of 
observable implicit flows.
%
We interpret the stack events, $push$ and $pop$, by updating the security 
stack $t$ (rule \textsc{\small stack}). We write $\circ$ to join the 
elements of a stack, i.e., $v \circ t$ is the result of pushing $v$ on top 
of stack $t$.
%
An $upgrade$ event increments the number $c_H$ of hidden implicit flows 
(rule \textsc{\small upgrade}).
%
Finally, note that $sink$ events are ignored while measuring micro flows; 
they are important for source-to-sink flows.

The last three columns of Figures~\ref{fig:traceBranchTaken} 
and~\ref{fig:traceBranchNotTaken} show the state of the iFlow interpreter 
after each trace event. In particular, the last three columns show the 
number of explicit, observable implicit, and hidden implicit flows, 
respectively.
%
In Figure~\ref{fig:traceBranchTaken}, Event~3 causes an explicit flow 
because it writes a tagged value into a fresh variable. Events~6 and~7 
happen while the tagged value $v_7$ is on the security stack, and therefore 
cause observable implicit flows.
In addition, Event~7 causes an explicit flow because the written value is 
tagged and overwrites a non-tagged value.
In total, the execution in Figure~\ref{fig:traceBranchTaken} has two 
explicit flows, two observable implicit flows, and no hidden implicit flow.
%
Figure~\ref{fig:traceBranchNotTaken} illustrates an execution where the 
branch is not taken. In contrast to Figure~\ref{fig:traceBranchTaken}, the 
upgrade event (Event~5) causes a hidden implicit flow.


\subsubsection{Source-to-Sink Flows}
\label{sec:S2SFlows}

To what degree do different kinds of flows contribute to policy violations?
To address this question, we consider transitive flows from a source of 
sensitive information to an untrusted sink, and analyze the micro flows that 
contribute to them. In the definitions presented in this section, upgrade 
statements are considered sources of sensitive information since they are 
points in a program where tagged values are produced from untagged
ones. At first, the approach computes a graph that represents how trace 
events depend on each other.

\begin{mydef}
The \textbf{event dependence graph} for an iFlow trace $T$ is a directed 
graph where
\begin{itemize}
  \item there is a node for each event in $T$,
  \item there exists an edge between two nodes $e_1$ and $e_2$ if and only 
    if $e_2$ uses a value that is produced by $e_1$.
\end{itemize}
\end{mydef}

The definition is based on two types of trace events: producers ($source$, 
$upgrade$, $operation$) and consumers ($operation$, $sink$, $push$, $write$, 
$upgrade$).
Our approach constructs the graph by a single pass through the trace.

Based on the event dependence graph, the approach extracts subtraces that 
contain all events that contribute to an information flow between a given 
source location $l_{src}$  and sink location $l_{snk}$.

\begin{mydef}
  \label{def:s2sLocationSubtrace}
  The \textbf{source-to-sink subtrace} for an event dependence graph $G$ and 
  two code locations $l_{src}$, $l_{snk}$ contains all trace events that are 
  part of a path in $G$ from an event $source(*,l_{src})$ (or $upgrade(*,*,l_{src})$) to an event 
  $sink(*,l_{snk})$, where $*$ means an arbitrary value.
\end{mydef}

Finally, we use the source-to-sink subtraces to measure which kinds of micro 
flows contribute to each individual violation of the policy.

For the example trace in Figure~\ref{fig:traceBranchTaken}, the 
source-to-sink event subtrace consists of all events in the trace, except 
for Event~7. The write performed by this event is irrelevant for the 
information flow between the source and the sink.

\subsection{Obtaining a Program with Upgrade Statements}
\label{sec:onlinePhase}

The approach described so far requires a program that indicates hidden 
implicit flows through upgrade statements.
To obtain such a program, we adapt a testing-based technique for 
automatically inserting upgrade statements~\cite{birgisson2012boosting}.
The basic idea is to repeatedly execute the program with a particular 
policy, to monitor the execution for potentially missed hidden implicit 
flows (using the PU monitoring strategy~\cite{austin2010permissive}, see 
Section~\ref{sec:background}), and to insert upgrade statements that avoid 
missing them.
Whenever the monitor terminates the program because it detects an access of 
a value $u$ that is marked as partially leaked, the approach modifies 
the program by inserting an upgrade statement at the code location where $u$ 
is used.
The process continues until it reaches a fixed point, i.e., until the 
program has enough upgrade statements for the given tests.

%%% MP: commenting for space reasons
%Our approach differs from Birgisson et al.'s work in several ways.
%First, we target the whole JavaScript language, whereas the existing 
%approach is evaluated with a Haskell prototype that targets a small core 
%language inspired by JavaScript.
%Second, we use the PU monitoring strategy, whereas the existing approach 
%uses NSU (Section~\ref{sec:background}). Our version of the PU strategy is 
%slightly more strict than~\cite{austin2010permissive}, reporting a violation 
%each time a read of the partially leaked data occurs, instead of only doing 
%so at branching, function calls and writes, as proposed in the original 
%form.




==> relatedWork.tex <==
\section{Related Work}
\label{sec:relatedwork}

Denning and Denning have pioneered in developing and formally describing 
information flow analyses~\cite{denning1977certification,Denning1976}.
In particular, Denning describes a simple language to abstract programs for
information flow analysis~\cite{Denning1976}. Our iFlow language shares the 
idea of abstraction but focuses on abstracting an execution instead of a 
program. A huge body of work has 
been created during the years to refine Denning's ideas and 
to adapt them to various programming languages.  In 
Table~\ref{tab:recent-work} presents some of the most recent approaches.

\paragraph*{Information Flow Analysis for JavaScript}
The omnipresence of JavaScript and potential security risks in 
JavaScript-based applications motivates various approaches on information 
flow analysis for JavaScript.
Chugh et al.\ propose a combined static-dynamic analysis that reports flows 
from code given to \code{eval()} to sensitive locations, such as the 
location bar of a site~\cite{chugh2009staged}.
%
Austin and Flanagan address the problem of hidden implicit 
flows~\cite{austin2009efficient,austin2010permissive}, as discussed in 
detail in Section~\ref{sec:background}.
Hedin et al.\ propose a dynamic analysis that implements the NSU strategy 
for a subset of JavaScript~\cite{Hedin2012}.
JSFlow supports the full JavaScript language, but it requires to insert 
upgrade statements manually~\cite{hedin2014jsflow}.
%
Birgisson et al.\ propose to  automatically 
insert upgrade statements~\cite{birgisson2012boosting} by iteratively 
executing a set of tests, which has inspired our methodology. Their approach 
is implemented for a JavaScript-like language, whereas we support the full 
JavaScript language.
%
Bichhawat et al.\ propose a dynamic information flow analysis 
that modifies the bytecode interpreter of a JavaScript 
engine~\cite{Bichhawat2014}. They describe a variant of the PU strategy, 
where the program is terminated whenever a partially leaked value may flow 
into the heap.

\paragraph*{Other Work on Information Flow Analysis}
Bao et al.\ show that considering implicit flows can cause a significant 
amount of false positives and propose a criterion to determine a subset of 
all conditionals to consider in an information flow analysis~\cite{Bao2010}.
Chandra et al.\ propose a \mbox{VM-based} analysis for Java that combines a 
conservative static analysis with a dynamic analysis to track all three 
kinds of flows considered in this paper~\cite{Chandra2007}.
Dytan is a dynamic information flow analysis for binaries that supports both 
explicit and observable implicit flows~\cite{Clause2007}.
Myers and Liskov~\cite{MyersL00} introduce Jif, a popular language for 
specifying security policies for Java programs that are further enforced 
statically.
A survey by Sabelfeld and Myers provides an overview of further static 
approaches to track information flows~\cite{Sabelfeld2003}.

\paragraph*{Applications of Information Flow Analysis}
Taint analysis and information flow analysis is widely used to discover 
potential vulnerabilities. All approaches we are aware of consider only a 
subset of the three kinds of flows studied in this paper.
%
Flax uses taint analysis to find incomplete or missing input validation and 
generates attacks that try to exploit the potential 
vulnerabilities~\cite{Saxena2010a}.
Lekies et al.\ propose a similar approach to detect DOM-based XSS 
vulnerabilities~\cite{Lekies2013}.
Jang et al.\ analyze various web sites with information flow policies 
targeted at common privacy leaks and attack vectors, such as cookie stealing 
and history sniffing~\cite{Jang2010}. Their analysis considers observable 
implicit flows but not hidden implicit flows.
Sabre analyzes flows inside browser extensions to discover malicious 
extensions~\cite{dhawan2009analyzing}. Their analysis considers only 
explicit flows.

\paragraph*{Studies of Information Flow}
King et al.~\cite{King2008} empirically study implicit flows detected by a 
static analysis. They report that most of the reported policy violations are 
false positives, mostly due to conservative handling of exceptions.
Our work focuses on dynamic analysis and addresses different questions that 
explore the advantages and disadvantages of considering different kinds of 
flows.
Another empirical study of information flows is by Masri et 
al.~\cite{masri2009measuring}. Their work studies how the length of flows 
(measured as the length of the static dependence chain), the strength of 
flows (measured based on entropy and correlations), and different kinds of 
information flows (explicit and observable implicit) relate to each other.
Similar to our methodology, Masri et al.\ build on a dynamic analysis.
Our work differs by addressing different research questions, a different 
language, and by considering hidden implicit flows, which are particularly 
relevant since recent research seeks ways to analyze them.





==> results.tex <==
\section{Empirical Study and Results}\label{sec:results}

\subsection{Subject Programs}

\label{sec:setup}
\begin{table}
  \caption{Subject programs, the number of used policies, the size of the program and the dynamic coverage achieved by our test suite.}
  \centering
  \setlength{\tabcolsep}{2.5pt}
  \renewcommand{\arraystretch}{0.8}
    \begin{tabular}{@{}rlrrr@{}}
	\toprule
  ID & Application & Policies& LoC & Branch \\
     &			   & 	& 	& Coverage\\
    \midrule
    1 	& alessioalex/ClientManager 	& 12	& 1,114 & 0.650\\
    2 	& andzdroid/mongo-express  		& 12	& 1,183 & 0.619\\
    3 	& ijin82/simple-node-blog 		& 12	& 2,031 & 0.604\\
    4 	& ccoenraets/nodecellar 		& 12	& 341 	& 0.500\\
    5 	& sergkr/swot 					& 12	& 1,699 & 0.577\\
    6 	& sanddudu/LightBlog 			& 12	& 989 	& 0.592\\
    7 	& contactkeala/lask 			& 12	& 320 	& 0.607\\
    8 	& docentkowalik/Roll-Call-App 	& 12	& 660 	& 0.521\\
    9 	& elizar/expressboard 			& 12	& 544 	& 0.638\\
    10 	& jpsoroulas/watcherjs 			& 12	& 3,635 & 0.630\\
    11 	& ddgarrett/mean-stack 			& 12	& 1,540 & 0.595\\
    12 	& Nekle/newsfeed 				& 12	& 445 	& 0.600\\
    %\iffalse app14 & \fi scottjason/retail-store-web & 129 & 15.01\% \\    
    \midrule
   	13 	& box2d 						& 980	& 10,844& 0.649\\	
 	14 	& crypto 						& 377	& 1,309 & 0.723\\	
	15 	& earley-boyer 					& 225	& 3,485 & 0.812\\ 	
	16 	& deltablue 					& 199	& 479 	& 0.811\\
	17 	& raytrace 						& 152	& 685 	& 0.706\\
	18 	& regexp 						& 258	& 1,795 & 0.991\\
	19 	& richards 						& 230 	& 304 	& 0.910\\
	20 	& splay 						& 200	& 237 	& 0.743\\

	

\midrule
		& Total 						& 2,765	& 33,639 & \\
  \bottomrule
  \end{tabular}
  \label{tab:apps}
\end{table}

We study \numberapps{} JavaScript programs that, in total over the entire 
study, yield over \lowerBoundEvents{} runtime events. Table~\ref{tab:apps} 
lists the subject programs, along with the number of security policies  
that we consider, the number of non-blank, non-comment lines of 
JavaScript source code, and the branch coverage of the analyzed executions.

Most of the study (RQ1 to RQ4) uses the programs listed in the upper part of 
the table. These programs are JavaScript server-side applications built on 
top of the popular Express framework (upper part of Table~\ref{tab:apps}).  
We select these programs for two reasons. First, being exposed to client 
requests, these programs naturally have security concerns. Second, these 
programs all have a client-side interface that enables us to exercise the 
programs with typical input. To execute the programs, we create automated 
browser tests\footnote{Based on Selenium, \url{http://www.seleniumhq.org/}.} 
that perform typical client-side usage scenarios.
%
We instrument the code of each program, excluding third-party 
libraries and the Express framework.

The lower part of Table~\ref{tab:apps} lists programs from Google's Octane 
benchmark, which we use to address RQ5. We select these programs because 
they come with inputs that exercise large parts of the code and because they 
are widely used JavaScript benchmark programs.
We exclude some benchmarks because they are not compatible with our 
node.js-based implementation.


\subsection{Information Flow Policies}

To address RQ1 to RQ4, we specify information flow policies for the programs 
in the upper part of Table~\ref{tab:apps}.
We consider reads from the file system, database accesses and incoming 
network requests as sources of sensitive information.
Furthermore, we consider writes to the file system, executing a child 
process, database accesses and sending a network response as untrusted sinks.
We combine these sources and sinks into \numberManualPolicies{} policies that cover 
realistic attack scenarios, such as server side command injection (flow from 
network request to child process), client side
command injection (flow from network request to network response), and 
sensitive data exposure (flow from filesystem to network response).
Of course, these policies do not ensure that all security concerns are 
covered and cannot guarantee that each flow corresponds to a security 
vulnerability.

\subsection{RQ1: Prevalence of Microflows}

\begin{figure}
\centering
\epsfig{file=results/gnuplot/prevalence-microflows.pdf, width=3.2in}
\caption{Prevalence of microflows. }
\label{fig:prevalenceRealistic}
\end{figure}

\iffalse
\begin{figure}
\centering
\epsfig{file=results/prevalenceSeeded.pdf, width=3.2in}
\caption{Prevalence of microflows in Experiment 2. }
\label{fig:prevalenceSeeded}
\end{figure}
\fi

At first, we address the question how prevalent explicit, observable 
implicit, and hidden implicit flows are among all operations that induce an 
information flow.

We execute each program with each of the 12 policies and consider only 
executions with at least one microflow. In Figure~\ref{fig:prevalenceRealistic}, we show averages across all executions.
The percentages in the figure correspond to the three counters $c_E$, $c_O$, 
and $c_H$ (Section~\ref{sec:metricsMicroFlows}). 

The figure shows that each program exposes both explicit and implicit flows.  
The majority of the implicit flows are observable implicit flows.
\numberappsImpFlow{} of the \numberappsRealistic{} programs also contain hidden implicit flows.  
Hidden implicit flows are less prevalent than observable implicit flows.

We draw several conclusions from these results.
First, all three kinds of flows occur in real-world programs. That is, an 
analysis that does not want to risk missing any flows must consider all 
three kinds.
%
Second, implicit flows are prevalent and are mostly dominated by observable 
implicit flows.
%
Third, the prevalence of different kinds of flows varies a lot between 
programs. That is, conclusions about the prevalence of particular kinds of 
flows that are drawn from one program may not be valid for other programs.



\subsection{RQ2: Contribution of Microflows to Policy Violations}
\label{sec:contribToViolations}

\begin{figure}
\centering
\epsfig{file=results/gnuplot/prevalence-microflows-e2e.pdf, width=3.4in}
\caption{Contribution of each type of microflow to violations of the 
policy.}
\label{fig:e2e-prev}
\end{figure}

%\begin{figure}
%\centering
%\epsfig{file=results/prevalence-e2e-manual.pdf, width=3.4in}
%\caption{Contribution of each type of microflow to violations of the 
%information flow policy for Experiment 1.}
%\label{fig:e2e-prevManual}
%\end{figure}

The following addresses the question to what degree microflows contribute to 
policy violations, i.e., to source-to-sink flows.
For example, a microflow may not contribute to any source-to-sink flow if 
the value that causes the microflow does not propagate to a sink.

We address this question in two ways.
First, we present the overall contribution of flows to violations as the 
prevalence of each kind of microflow in source-to-sink subtraces.
We consider only traces that contain at least one source-to-sink flow, which 
yields 7 of the \numberappsRealistic{} programs.
%
Figure~\ref{fig:e2e-prev} summarizes the 
results. Each column shows the average percentage of each type of microflow 
that is involved in a policy violation. Explicit flows and observable 
implicit flows contribute most to source-to-sink flows.

As a second way to address RQ2, we analyze which kinds of microflows are 
essential in detecting particular policy violations.
We consider source-to-sink subtraces of all executions that contain 
at least one policy violation.
Each considered subtrace consists of a single source-to-sink flow.
We analyze all the types of microflows that appear and classify subtraces 
based on their microflows.

\begin{figure}
\centering
\epsfig{file=results/gnuplot/diff-types-e2e-bar.pdf, width=3.2in}
\caption{Distribution of different types of source-to-sink flows.}
\label{fig:diff-types}
\end{figure}

Figure~\ref{fig:diff-types} shows the result of this classification. We make 
three observations:
\begin{itemize}
  \item The two largest categories of violations can be detected by a 
    lightweight taint analysis. Policy violations where secret information 
    is propagated only via explicit flows account for 30\% of all 
    violations.
    The ``no microflows'' category, which means a direct transfer of data 
    from source to sink, accounts for 42.5\% of the violations.
  \item Two other relatively large categories of violations may be missed by 
    a taint analysis but will be detected by an information flow analysis 
    that maintains a security stack: Violations that involve both explicit 
    and observable implicit flows (15\%), and violations caused exclusively 
    by observable implicit flows (10\%).
  \item Finally, some of the violations are caused only by hidden implicit 
    flows (2.5\%). Detecting such violations requires a sophisticated 
    analysis, e.g., based on upgrade 
    statements~\cite{Austin2009,austin2010permissive}.
\end{itemize}

In summary, we draw the following conclusions from the results for RQ2.
First, a lightweight analysis that focuses on explicit flows, such as a 
taint analysis, covers a significant percentage of all policy violations.  
That is, such analyses are a valid choice as a first layer of security 
because they can reveal various problems at a relatively low cost.
At the same time, a taint analysis also misses a significant percentage of 
policy violations, underlining the need for stronger analyses.
%
Second, analyses that consider both explicit and observable implicit flows 
observe the majority of all policy violations. For example, such an analysis 
would detect more than 90\% of the violations we observe.
%
Third, a small but non-negligible percentage of policy violations can only 
be detected by an analysis that also considers hidden implicit flows. That 
is, ignoring hidden implicit flows leads to missed policy violations, which, 
in the worst case, may mean that an attack or a vulnerability remains 
unnoticed.


\subsection{RQ3: Importance of Data Propagated through Implicit Flows}
\label{sec:importanceOfIF}

The following addresses the question whether implicit flows that cause 
policy violations propagate important data. The importance of data depends 
on the application and on the policy that the developers want to enforce.
%
We manually inspect a sample of all code locations that trigger 
source-to-sink flows involving implicit flows. Initially, we randomly select 
and inspect 15 code locations with implicit flows, and later inspect 
additional 11 code locations with implicit flows of a particular kind.

\begin{figure}
\begin{spacing}{0.9}
\begin{lstlisting}
function (markSource(req), res)   {/*#\label{line:markFct}#*/
  if (req.user) {
    res.redirect('/threads');
  }
  res.render('index', {
    url: req.url,
    errorFlash: req.flash('error'),/*#\label{line:Hcall1}#*/
    successFlash: req.flash('info')/*#\label{line:Hcall2}#*/
  });
};
\end{lstlisting}
\end{spacing}
\caption{Example of implicit flow due to function calls, taken from elizar/expressboard. }
\label{fig:fctif}
\end{figure}

The main root cause of implicit flows are calls to $H$-labeled functions (13 
of 15 flows). Since JavaScript supports higher-order functions, the decision 
to which function a call resolves may implicitly propagate sensitive 
information~\cite{Hedin2012}. To detect such flows, the analysis allows for 
marking function objects as secret and records an observable implicit flow 
whenever an $H$-labeled function gets called.
%
Figure~\ref{fig:fctif} gives an example of a flow caused by an $H$-labeled 
function. The security policy recursively marks the \code{req} object, which 
represents an incoming request from the network, as secret 
(line~\ref{line:markFct}).
As a result, calls to \code{req.flash()} (lines~\ref{line:Hcall1} 
and~\ref{line:Hcall2}) induce an implicit flow.
%
Even though a higher-order function can, in principle, convey sensitive 
information, we find that none of the examples we inspect do so.

Based on the above finding, we ignore implicit flows caused by $H$-labeled 
functions and further inspect the remaining implicit flows.
Many dynamic instances of implicit flows are caused by the same source code 
location, and the remaining implicit flows boil down to eleven distinct code 
locations, allowing us to inspect all of them.
%In theory, every implicit flow leaks one bit of information, namely the 
%conditional's value.
To determine the practical value of the propagated information, we analyze 
several aspects of each implicit flow location.

\paragraph*{Kind of conditional}
The conditionals that cause implicit flows perform four kinds of checks:
\begin{itemize*}
\item 4 of 11 are value checks, e.g. \code{if (a !== c)}.
\item 3 of 11 are existence checks, e.g. \code{if (a)}.
\item 2 of 11 are type checks, e.g. \code{if (typeof a === c)}.
\item 2 of 11 are a combination of multiple other kinds.
\end{itemize*}
Intuitively, value checks have the highest chance to propagate a significant 
amount of information because they may convey the entire value of a secret 
variable.

\paragraph*{Strict control dependence}
3 of 11 locations with implicit flows are strict control 
dependences~\cite{bao2010strict}. This special type of implicit flow 
completely reveals the value of a secret variable, e.g., by checking that 
a variable is equal to a constant.

\paragraph*{Variables in conditional}
The number of variables involved in a conditional influences the strength of 
the information flow. If there are more variables involved, it is harder to 
reconstruct individual pieces of information about each variable.
We find that almost all (10 of 11) of the conditionals that cause implicit 
flows involve only a single variable.

\paragraph*{Variables written in the branches}
The number of variables that are written in a secret context varies between 
1 and 4 (median: 2). Only for three code locations, some of these variables 
are written in both branches. This result suggests that most code locations 
that cause implicit flows may cause hidden implicit flows.


%In Table~\ref{tab:manual-analysis}, we report the results of our manual 
%inspection with respects to each of the presented dimensions.
%
%\begin{table*}
%  \small
%  \setlength{\tabcolsep}{3pt}
%    \begin{tabular}{@{}lccccc@{}}
%	\toprule
%  Location & Variables in conditional & Modified variables & Modified on both branches & Type of conditional & Strict Control Dependence \\
%    \midrule
%    ddgarrett/mean-stack & 1 & 4 & 1 & C1  & yes  \\
%    ddgarrett/mean-stack & 1 & 3 & 0 & C1  & yes  \\
%	ijin82/simple-node-blog & 1 & 2 & 2 & C1 & no \\ 
%    andzdroid/mongo-express & 1 & 2 & 1 & C2 & no \\ 
%    ddgarrett/mean-stack & 1 & 2 & 0 & C4=C1+C2 & yes \\ 
%    ddgarrett/mean-stack & 1 & 2 & 0 & C2 & no \\ 
%    ddgarrett/mean-stack & 1 & 1 & 0 & C3 & no \\ 
%    ddgarrett/mean-stack & 1 & 1 & 0 & C2 & no \\
%    ddgarrett/mean-stack & 2 & 2 & 0 & C4=C2+C2 & no \\
%    ddgarrett/mean-stack & 1 & 1 & 0 & C3 & no \\
%    andzdroid/mongo-express & 1 & 1 & 0 & C1 & no \\
%	\bottomrule
%  \end{tabular}
%  \caption{Results of our manual analysis.}
%  \label{tab:manual-analysis}
%\end{table*}

Beyond these observations, the most important question is whether the 
implicit flows cause any security vulnerabilities.
We find that, to the best of our knowledge, none of the implicit flows we 
inspect cause a security problem.
Most of the implicit flows are harmless and do not convey much information 
(e.g. type checks, existence checks) and the ones that propagate important 
information cannot be exploited as they are not close to a sink.
In other words, even though the information flow policies are technically 
violated, a security analyst would consider these violations as false 
positives.

Our findings suggest that implicit flows are less important than explicit 
flows because they often do not convey significant amount of information.
%
However, it is important to keep in mind that our study focuses on 
non-malicious code, which is unlikely to violate reasonable information flow 
policies. In contrast, malicious code may try to hide its activities in a 
sequence of implicit flows.


\subsection{RQ4: Cost of Considering Implicit Flows}

We address the question what costs considering implicit flows involves in 
three ways.
%
First, we approximate the computational cost of tracking implicit flows at 
runtime as the number of runtime operations that an analysis considers.
We consider a full fledged information flow analysis as the baseline and 
compute how many runtime operations a more lightweight analysis would 
ignore.
To compute the reduction achieved by ignoring implicit flows, we consider 
the event dependence graph of all source-to-sink flows and remove all events 
that impose implicit flows as well as events transitively caused only by 
these events. We ignore $source$ and $sink$ events when computing the trace 
size because these events are not relevant for propagating how secret 
information flows through the program.

\begin{figure}[t]
\centering
\epsfig{file=results/gnuplot/trace-reduction.pdf, width=3.2in}
\caption{Trace size reduction when not considering implicit flows.}
\label{fig:trace-shrinkage}
\end{figure}

Figure~\ref{fig:trace-shrinkage} shows to what degree ignoring implicit 
flows reduces the number of runtime operations to consider. The figure shows 
the percentage of trace events that can be ignored for each source-to-sink 
violation.
On average, the number of relevant runtime operations decreases by 
\percEventsExplicitOnly{}.
Some source-to-sink violations even completely disappear (as we also show in 
Section~\ref{sec:contribToViolations}), effectively reducing the trace size 
by 100\%.
We conclude that ignoring implicit flows significantly reduces the overhead 
imposed by an information flow analysis.

Second, we approximate the human cost of inspecting potential security 
problems as the number of distinct code locations that a security analyst 
must consider when inspecting implicit flows. As reported in 
Section~\ref{sec:importanceOfIF}, the number of distinct locations that 
cause an implicit flow is relatively low,
%% excluding calls to secret functions; ideally, we should also count those
which enables manual inspection of these locations in reasonable time. Therefore, 
a security analyst can manually inspect suspicious flows to see if 
they are vulnerabilities.

Third, we study the cost of adding upgrade statements to a program, which is 
a prerequisite for using state of the art dynamic analyses that consider
hidden implicit flows~\cite{austin2009efficient,austin2010permissive}.
We expect that, in a realistic usage scenario, at least some upgrade 
statements will be added manually, i.e., impose some human cost.
While the automated insertion of upgrade statements avoids this cost, it is 
limited by the coverage of tests used during the insertion process, and 
therefore unlikely to insert all required upgrades.
Based on the automatically inserted upgrade statements, we find that, for 
most of the applications, no upgrades or a low number of upgrades is 
required. However, some applications require more than 30 upgrades, and 
inserting these manually seems impractical because the security analyst 
needs to understand the context for each individual upgrade.
We conclude that the cost of inserting upgrades may be manageable for some 
applications but can easily become a major obstacle for adopting a dynamic 
information flow analysis that considers hidden implicit flows.

%\begin{figure}[t]
%\centering
%\epsfig{file=results/number-upgrades.png, width=3.2in}
%\caption{Inserted upgrades for each run.}
%\label{fig:number-upgrades}
%\end{figure}


\subsection{RQ5: Influence of the Policy on the Observed Kinds of 
Microflows}

The following addresses the question to what degree the information flow 
policy influences the prevalence of different kinds of flows.
To study this question, we automatically insert a large number of different 
policies into programs and measure the prevalence of flows for each policy.
For this research question, we use the Octane benchmark programs, listed in 
the lower part of Table~\ref{tab:apps}. The rational for using these 
programs is that they are more suitable for automatically inserting and 
analyzing many policies, because they can be easily executed many times and 
because the provided benchmark inputs provide high code coverage.

Our algorithm for seeding a policy identifies all literals and functions in 
the program and randomly picks one as the source. Then, it marks a random 
subset (20\%) of all functions in the program as sinks. The algorithm 
automatically embeds policies into programs via AST rewriting.
We create multiple sinks per policy to increase the chance to observe a 
source-to-sink flow in a particular execution.
Since the policy seeding algorithm depends on random decisions, we 
repeatedly seed policies into each program and perform all measurements with 
a set of different policies.
In total, we seed and check more than 2,500 security policies.
%
%We consider for each program 20 random policies that yield a source-to-sink 
%subtrace.
%
For performance reasons, we use a more lightweight implementation of the 
information flow analysis than for the other research questions, which does 
not consider native calls. Most of the Octane benchmarks do not have such 
calls.


\iffalse
\begin{enumerate}
  \item Parse the program into an AST.
  \item Identify all literals and functions defined in the program and randomly
pick one of them, called $s$.
  \item Mark $s$ as a source of confidential information.
  \item Identify all functions defined in the program and randomly select a 
    subset $F$ of them. Add each function to $F$ with a 
    configurable probability $p_{sink}$. Unless otherwise specified, we use 
    $p_{sink}=0.2$ as default.
  \item Mark all functions in $F$ as a sink.
  \item Generate JavaScript code from the modified AST.
\end{enumerate}
\fi


\begin{figure}
\centering
\epsfig{file=results/gnuplot/box-and-wiskers.pdf, width=3.2in}
\caption{Influence of the policy on the prevalence of each type of flow.  
The box shows the 25\% and 75\% percentiles and the bold lines mark the median values.}
\label{fig:infl-policy}
\end{figure}

Figure~\ref{fig:infl-policy} shows how much the distribution of microflows
varies depending on the policy.
The figure summarizes for each program the percentage of the three kinds of 
flows: The vertical show the range between the minimum and the maximum 
observed values; the boxes show the 25\% and 75\% percentiles.  The results 
show that the choice of the policy has a large impact on the existence of 
these types of flows.

We draw two conclusions from these results.
First, a developer or security analyst may deliberately choose a lightweight 
analysis because it seems sufficient for the current policy. However, our 
results show that it is important to reconsider this decision when changing the 
policy, because a different policy may expose different flows, even for the 
same program.
%
Second, there is potential for future work on identifying policies for which 
a lightweight analysis provides sufficiently strong security guarantees.  
Such a technique could help security analysts to handle the cost-benefit 
tradeoff of information flow analysis.





\subsection{Threats to Validity}

The validity of the conclusions drawn from our study are subject to several 
threats.
First, our dynamic information flow analysis uses a simple model for native 
functions (Section~\ref{sec:implementation}), which may not accurately 
describe all effects of these functions. To minimize the influence of this 
limitation, we focus the study on subject programs that have relatively few 
native calls and that do not, e.g., interact with the DOM.
Second, our results are limited to the programs we consider and may not 
generalize to other programs or classes of programs. In particular, we only 
consider non-malicious programs, where difficult to analyze flows may be 
less prevalent than in malicious code. Our methodology is generic enough to 
be easily applied to other programs.
Finally, the hidden implicit flows that our methodology can observe are 
bounded by the upgrade statements inserted into the programs, which in turn 
depend on the tests we use to exercise the programs 
(Section~\ref{sec:onlinePhase}). To mitigate this threat we constructed the 
automated tests in a way that the dynamic coverage is increased. However, 
multiple paths cannot be covered due to a variety of factors: double validation 
on client side and server side, error cases that cannot be triggered from 
client side or unfeasible execution paths.
%
Despite these limitations, our study produces interesting insights about the 
kinds of flows that appear in real-world JavaScript programs and the 
cost-benefit tradeoff of information flow analysis.



==> summarytable.tex <==
\begin{table*}
  \caption{Insecure programs grouped by category, showing security policies,
    total programs size, average sensitive branch coverage and total number of
    upgrades. See Table~\ref{tab:apps} for more details.}
  \footnotesize
  \renewcommand{\arraystretch}{0.9}
  \centering
  \setlength{\tabcolsep}{5.5pt}
\def\arraystretch{0.8}%
    \begin{tabular}{@{}p{1.5cm}p{11cm}rrrc@{}}
	\toprule
Category & Policy & No. Programs & LoC & SBC &Upgs \\
\midrule
Injections & {\bfseries Sources} = \{module's interface, file system, network
traffic\};
{\bfseries Sinks} = \{eval, exec\} & 19 & 24,497 & 0.80 & 32 \\
ReDoS  & {\bfseries Sources} = \{module's interface\}; {\bfseries Sinks} =
\{APIs matching regular expressions\} & 20 & 18,021 & 0.71 & 6\\
Buffer  & {\bfseries Sources} = \{APIs reading uninitialized buffers\};
{\bfseries Sinks} =
\{network
traffic, module's interface\} &7 & 5,648 & 0.69 & 4 \\
Client-Side  & {\bfseries Sources} = \{Properties of HTMLElement such as color
or offset, onload event, doNotTrack flag\}; {\bfseries Sinks} = \{img.src,
request.open, console.log, HTMLelement.innerHTML\}  & 10 & 2236 &
0.35 & 10\\
    \bottomrule
    \end{tabular}
    \label{tab:summary}
\end{table*}

